Prospects for the characterization of the VHE emission from the Crab Nebula and Pulsar with the Cherenkov Telescope Array

The Cherenkov Telescope Array (CTA) will be the next generation instrument for the very high energy gamma-ray astrophysics domain. With its enhanced sensitivity in comparison with the current facilities, CTA is expected to shed light on a varied population of sources. In particular, we will achieve a deeper knowledge of the Crab nebula and pulsar, which are the best characterized pulsar wind nebula and rotation powered pulsar, respectively. We aim at studying the capabilities of CTA regarding these objects through simulations, using the main tools currently in development for the CTA future data analysis: Gammapy and ctools. We conclude that, even using conservative Instrument Response Functions, CTA will be able to resolve many uncertainties regarding the spectrum and morphology of the pulsar and its nebula. The large energy range covered by CTA will allow us to disentangle the nebula spectral shape among different hypotheses, corresponding to different underlying emitting mechanisms. In addition, resolving internal structures (smaller than ~ 0.02 degrees in size) in the nebula and unveiling their location, would provide crucial information about the propagation of particles in the magnetized medium. We used a theoretical asymmetric model to characterise the morphology of the nebula and we showed that if predictions of such morphology exist, for instance as a result of hydrodynamical or magneto-hydrodynamical simulations, it can be directly compared with CTA results. We also tested the capability of CTA to detect periodic radiation from the Crab pulsar obtaining a precise measurement of different light curves shapes.

==> bib.tex <==
@ARTICLE{MILAGRO_CRAB,
       author = {{Abdo}, A.~A. and {Allen}, B.~T. and {Atkins}, R. and {Aune}, T. and
         {Benbow}, W. and {Berley}, D. and {Blaufuss}, E. and {Bonamente}, E. and
         {Bussons}, J. and {Chen}, C.},
        title = "{Observation and Spectral Measurements of the Crab Nebula with Milagro}",
      journal = {\apj},
     keywords = {acceleration of particles, astroparticle physics, gamma rays: general, pulsars: individual: Crab Pulsar, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2012",
        month = "May",
       volume = {750},
       number = {1},
          eid = {63},
        pages = {63},
          doi = {10.1088/0004-637X/750/1/63},
archivePrefix = {arXiv},
       eprint = {1110.0409},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...750...63A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{HAWC_CRAB,
       author = {{Abeysekara}, A.~U. and {Albert}, A. and {Alfaro}, R. and {Alvarez}, C. and
         {{\'A}lvarez}, J.~D. and {Arceo}, R. and
         {Arteaga-Vel{\'a}zquez}, J.~C. and {Ayala Solares}, H.~A. and
         {Barber}, A.~S. and {Bautista-Elivar}, N.},
        title = "{Observation of the Crab Nebula with the HAWC Gamma-Ray Observatory}",
      journal = {\apj},
     keywords = {acceleration of particles, gamma rays: general, ISM: individual objects: Crab Nebula, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Jul",
       volume = {843},
       number = {1},
          eid = {39},
        pages = {39},
          doi = {10.3847/1538-4357/aa7555},
archivePrefix = {arXiv},
       eprint = {1701.01778},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...843...39A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{CTA_sys,
  author = {{CTA}, collaboration},
  journal = {CTA System-Level Science Performance Requirements.},
  adsurl = {https://www.cta-observatory.org/wp-content/uploads/2019/04/CTA-SPE-SCI-00000-0001_Issue_1_SystemLevelSciencePerformanceReqs.pdf},
  year = 2018
}
@ARTICLE{1979Efron,
   author = {{Efron}, B.},
    title = "{Bootstrap Methods: Another Look at the Jackknife}",
  journal = {Annals of Statistics},
     year = 1979,
   volume = 7,
   number = {1},
    pages = {1-26},
     doi = {10.1214/aos/1176344552},
}

@article{Contopoulos:1999,
      author         = "Contopoulos, Ioannis and Kazanas, Demosthenes and Fendt,
                        Christian",
      title          = "{The axisymmetric pulsar magnetosphere}",
      journal        = "Astrophys. J.",
      volume         = "511",
      year           = "1999",
      pages          = "351",
      doi            = "10.1086/306652",
      eprint         = "astro-ph/9903049",
}

@ARTICLE{1979Cash,
   author = {{Cash}, W.},
    title = "{Parameter estimation in astronomy through application of the likelihood ratio}",
  journal = {Astrophysical Journal},
     year = 1979,
    month = mar,
   volume = 228,
    pages = {939-947},
      doi = {10.1086/156922},
}

@ARTICLE{1976KU,
   author = {{Ku}, W. and {Kestenbaum}, H.~L. and {Novick}, R. and {Wolff}, R.~S.
	},
    title = "{Energy dependence of the size of the X-ray source in the Crab Nebula}",
  journal = {Astrophysical Journal},
 keywords = {Crab Nebula, Energy Distribution, X Ray Astronomy, X Ray Sources, Cosmic Dust, Electron Distribution, X Ray Density Measurement, X Ray Scattering, X Ray Spectra},
     year = 1976,
    month = mar,
   volume = 204,
    pages = {L77-L81},
      doi = {10.1086/182058},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...204L..77K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010DeJagger,
   author = {{De Jager}, O.~C. and {B{\"u}sching}, I.},
    title = "{The H-test probability distribution revisited: improved sensitivity}",
  journal = {Astronomy and Astrophysics},
archivePrefix = "arXiv",
   eprint = {1005.4867},
 primaryClass = "astro-ph.HE",
 keywords = {methods: statistical, pulsars: general},
     year = 2010,
    month = jul,
   volume = 517,
      eid = {L9},
    pages = {L9},
      doi = {10.1051/0004-6361/201014362},
}

@ARTICLE{1989DeJagger,
   author = {{De Jager}, O.~C. and {Raubenheimer}, B.~C. and {Swanepoel}, J.~W.~H.
	},
    title = "{A poweful test for weak periodic signals with unknown light curve shape in sparse data}",
  journal = {Astronomy and Astrophysics},
     year = 1989,
    month = aug,
   volume = 221,
    pages = {180-190},
}

@ARTICLE{2004Rots,
   author = {{Rots}, A.~H. and {Jahoda}, K. and {Lyne}, A.~G.},
    title = "{Absolute Timing of the Crab Pulsar with the Rossi X-Ray Timing Explorer}",
  journal = {The Astrophysical Journal},
   eprint = {astro-ph/0403187},
 keywords = {Stars: Pulsars: Individual: Name: Crab Pulsar, X-Rays: Stars},
     year = 2004,
    month = apr,
   volume = 605,
    pages = {L129-L132},
      doi = {10.1086/420842},
}

@ARTICLE{2008Volpi,
   author = {{Volpi}, D. and {Del Zanna}, L. and {Amato}, E. and {Bucciantini}, N.
	},
    title = "{Non-thermal emission from relativistic MHD simulations of pulsar wind nebulae: from synchrotron to inverse Compton}",
  journal = {Astronomy and Astrophysics},
     year = 2008,
    month = jul,
   volume = 485,
    pages = {337-349},
      doi = {10.1051/0004-6361:200809424},
}


@ARTICLE{2012Aleksic,
   author = {{Aleksi{\'c}}, J. and others
	},
    title = "{Phase-resolved energy spectra of the Crab pulsar in the range of 50-400 GeV measured with the MAGIC telescopes}",
  journal = {Astronomy and Astrophysics},
   year = 2012,
  month = apr,
  volume = 540,
  eid = {A69},
  pages = {A69},
  doi = {10.1051/0004-6361/201118166},
}


@ARTICLE{2008Kaplan,
   author = {{Kaplan}, D.~L. and {Chatterjee}, S. and {Gaensler}, B.~M. and 
	{Anderson}, J.},
    title = "{A Precise Proper Motion for the Crab Pulsar, and the Difficulty of Testing Spin-Kick Alignment for Young Neutron Stars}",
  journal = {The Astrophysical Journal},
archivePrefix = "arXiv",
   eprint = {0801.1142},
     year = 2008,
    month = apr,
   volume = 677,
    pages = {1201-1215},
      doi = {10.1086/529026},

}

@ARTICLE{2011Abdo,
   author = {{Abdo}, A.~A. and others},
    title = "{Gamma-Ray Flares from the Crab Nebula}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1011.3855},
 primaryClass = "astro-ph.HE",
     year = 2011,
    month = feb,
   volume = 331,
    pages = {739},
      doi = {10.1126/science.1199705},
}


@ARTICLE{2001Piron,
   author = {{Piron}, F. and others},
    title = "{Temporal and spectral gamma-ray properties of Mkn 421 above 250 GeV from CAT observations between 1996 and 2000}",
  journal = {Astronomy and Astrophysics},
   eprint = {astro-ph/0106196},
     year = 2001,
    month = aug,
   volume = 374,
    pages = {895-906},
      doi = {10.1051/0004-6361:20010798},
}

@ARTICLE{Aharonian2006,
   author = {{Aharonian}, F. and others},
    title = "{Observations of the Crab nebula with HESS}",
  journal = {Astronomy and Astrophysics},
   eprint = {astro-ph/0607333},
 keywords = {gamma rays: observations, ISM: individual objects: Crab, nebula, ISM: supernova remnants},
     year = 2006,
    month = oct,
   volume = 457,
    pages = {899-915},
      doi = {10.1051/0004-6361:20065351},
}

@ARTICLE{2016Ambrogi,
   author = {{Ambrogi}, L. and {De O{\~n}a Wilhelmi}, E. and {Aharonian}, F.
	},
    title = "{On the potential of atmospheric Cherenkov telescope arrays for resolving TeV gamma-ray sources in the Galactic plane}",
  journal = {Astroparticle Physics},
   eprint = {1603.04365},
     year = 2016,
    month = jul,
   volume = 80,
    pages = {22-33},
      doi = {10.1016/j.astropartphys.2016.03.004},
}
@ARTICLE{1996Atoyan,
   author = {{Atoyan}, A.~M. and {Aharonian}, F.~A.},
    title = "{On the mechanisms of gamma radiation in the Crab Nebula}",
  journal = {Monthly Notices of the Royal Astronomical Society},
 keywords = {RADIATION MECHANISMS: NONTHERMAL, ISM: INDIVIDUAL: CRAB NEBULA, GAMMA-RAYS: THEORY},
     year = 1996,
    month = jan,
   volume = 278,
    pages = {525-541},
      doi = {10.1093/mnras/278.2.525},
}
@ARTICLE{2016Burtovoi,
   author = {{Burtovoi}, A. and {Zampieri}, L.},
    title = "{Simulated gamma-ray pulse profile of the Crab pulsar with the Cherenkov Telescope Array}",
  journal = {Monthly Notices of the Royal Astronomical Society},
   eprint = {1604.04066},
     year = 2016,
    month = jul,
   volume = 459,
    pages = {3783-3791},
      doi = {10.1093/mnras/stw883},
}

@ARTICLE{2009Pellizzoni,
   author = {{Pellizzoni}, A. and others},
    title = "{High-Resolution Timing Observations of Spin-Powered Pulsars with the AGILE Gamma-Ray Telescope}",
  journal = {The Astrophysical Journal},
   eprint = {0810.1516},
     year = 2009,
    month = feb,
   volume = 691,
    pages = {1618-1633},
      doi = {10.1088/0004-637X/691/2/1618},
}

@ARTICLE{Molkov2009,
author = {Molkov, Serge and Jourdain, E and P. Roques, J},
year = {2009},
month = {11},
pages = {},
title = {Absolute timing of the Crab pulsar with the INTEGRAL/SPI telescope},
volume = {708},
journal = {The Astrophysical Journal}
}

@ARTICLE{2008Oosterbroek,
   author = {{Oosterbroek}, T. and {Cognard}, I. and {Golden}, A. and {Verhoeve}, P. and 
	{Martin}, D.~D.~E. and {Erd}, C. and {Schulz}, R. and {St{\"u}we}, J.~A. and 
	{Stankov}, A. and {Ho}, T.},
    title = "{Simultaneous absolute timing of the Crab pulsar at radio and optical wavelengths}",
  journal = {Astronomy and Astrophysics},
archivePrefix = "arXiv",
   eprint = {0806.3634},
 keywords = {stars: pulsars: individual: Crab Pulsar, PSR J0534+2200},
     year = 2008,
    month = sep,
   volume = 488,
    pages = {271-277},
      doi = {10.1051/0004-6361:200809751},
}

@ARTICLE{2003Kuiper,
   author = {{Kuiper}, L. and {Hermsen}, W.},
    title = "{X-ray and gamma-ray observations of millisecond pulsars}",
  journal = {ArXiv Astrophysics e-prints},
   eprint = {astro-ph/0312204},
 keywords = {Astrophysics},
     year = 2003,
    month = dec,
   adsurl = {http://adsabs.harvard.edu/abs/2003astro.ph.12204K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2010Abdo,
   author = {{Abdo}, A.~A. and others},
    title = "{Fermi Large Area Telescope Observations of the Crab Pulsar And Nebula}",
  journal = {The Astrophysical Journal},
     year = 2010,
    month = jan,
   volume = 708,
    pages = {1254-1267},
      doi = {10.1088/0004-637X/708/2/1254},
}

@ARTICLE{1973Trimble,
   author = {{Trimble}, V.},
    title = "{The Distance to the Crab Nebula and NP 0532}",
  journal = {Publications of the Astronomical Society of the Pacific},
     year = 1973,
    month = oct,
   volume = 85,
    pages = {579},
      doi = {10.1086/129507},
 }
@ARTICLE{2008CTAIRFs,
   author = {{Bernl{\"o}hr}, K.},
    title = "{Simulation of imaging atmospheric Cherenkov telescopes with CORSIKA and sim\_ telarray}",
  journal = {Astroparticle Physics},
archivePrefix = "arXiv",
   eprint = {0808.2253},
 keywords = {Applications of Monte Carlo methods, Computer modeling and simulation, X- and gamma-ray telescopes and instrumentation},
     year = 2008,
    month = oct,
   volume = 30,
    pages = {149-158},
      doi = {10.1016/j.astropartphys.2008.07.009},
   adsurl = {http://adsabs.harvard.edu/abs/2008APh....30..149B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{NEDMEAD1,
author = {Lagarias, Jeffrey and A. Reeds, James and H. Wright, Margaret and Wright, Paul},
year = {1998},
month = {12},
pages = {112-147},
title = {Convergence Properties of the Nelder--Mead Simplex Method in Low Dimensions},
volume = {9},
journal = {SIAM Journal on Optimization}
}

@inbook{NEADMED2,
title = "Direct search methods: Once scorned, now respectable",
author = "Margaret Wright",
year = "1996",
language = "English (US)",
pages = "191--208",
journal = "Numerical analysis",
publisher = "Addison-Wesley",
}

@ARTICLE{2012NatureAharonian,
   author = {{Aharonian}, F.~A. and {Bogovalov}, S.~V. and {Khangulyan}, D.
	},
    title = "{Abrupt acceleration of a `cold' ultrarelativistic wind from the Crab pulsar}",
  journal = {Nature},
     year = 2012,
    month = feb,
   volume = 482,
    pages = {507-509},
      doi = {10.1038/nature10793},
   adsurl = {http://adsabs.harvard.edu/abs/2012Natur.482..507A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015Mochol,
   author = {{Mochol}, I. and {P{\'e}tri}, J.},
    title = "{Very high energy emission as a probe of relativistic magnetic reconnection in pulsar winds}",
  journal = {Monthly Notices of the Royal Astronomical Society},
archivePrefix = "arXiv",
   eprint = {1501.07123},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, magnetic fields, magnetic reconnection, radiation mechanisms: non-thermal, pulsars: general, gamma-rays: stars},
     year = 2015,
    month = apr,
   volume = 449,
    pages = {L51-L55},
      doi = {10.1093/mnrasl/slv018},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.449L..51M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011Aleksic,
   author = {{Aleksi{\'c}}, J. and others},
    title = "{Observations of the Crab Pulsar between 25 and 100 GeV with the MAGIC I Telescope}",
  journal = {The Astrophysical Journal},
   eprint = {1108.5391},
     year = 2011,
    month = nov,
   volume = 742,
      eid = {43},
    pages = {43},
      doi = {10.1088/0004-637X/742/1/43},
}

@ARTICLE{1973Mcbreen,
   author = {{McBreen}, B. and {Ball}, Jr., S.~E. and {Campbell}, M. and 
	{Greisen}, K. and {Koch}, D.},
    title = "{Pulsed high-energy gamma rays from the Crab nebula.}",
  journal = {\apj},
     year = 1973,
    month = sep,
   volume = 184,
    pages = {571-580},
}

@INPROCEEDINGS{1996Eikenberry,
   author = {{Eikenberry}, S.~S. and {Fazio}, G.~G.},
    title = "{The Infrared to Gamma-Ray Pulse Shape of the Crab Nebula Pulsar}",
  journal = {The Astrophysical Journal},
   eprint = {astro-ph/9607120},
 keywords = {Stars: Pulsars: Individual: Alphanumeric: PSR 0531+21, Radiation Mechanisms: Nonthermal, Stars: Neutron},
     year = 1997,
    month = feb,
   volume = 476,
    pages = {281-290},
      doi = {10.1086/303616},
}

@INPROCEEDINGS{2017Zanin,
   author = {{Zanin}, R.},
    title = "{The Crab pulsar at VHE}",
booktitle = {European Physical Journal Web of Conferences},
     year = 2017,
   series = {European Physical Journal Web of Conferences},
   volume = 136,
archivePrefix = "arXiv",
   eprint = {1701.07364},
 primaryClass = "astro-ph.HE",
    month = mar,
      eid = {03003},
    pages = {03003},
      doi = {10.1051/epjconf/201713603003},
}

@ARTICLE{2011ScienceVeritas,
   author = {{Aliu}, E. and others},
    title = "{Detection of Pulsed Gamma Rays Above 100 GeV from the Crab Pulsar}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {1108.3797},
 primaryClass = "astro-ph.HE",
     year = 2011,
    month = oct,
   volume = 334,
    pages = {69},
      doi = {10.1126/science.1208192},
}

@ARTICLE{Sys1,
   author = {{Maccarone}, M.~C. and {Parsons}, D. and {Gaug}, M. and {de los Reyes}, R. and 
	{CTA Consortium}, f.~t.},
    title = "{Tools and Procedures for the CTA Array Calibration}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1709.03081},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2017,
    month = sep,
}

@ARTICLE{Sys2,
   author = {{Silverwood}, H. and {Weniger}, C. and {Scott}, P. and {Bertone}, G.
	},
    title = "{A realistic assessment of the CTA sensitivity to dark matter annihilation}",
  journal = {Journal of Cosmology and Astroparticle Physics},
archivePrefix = "arXiv",
   eprint = {1408.4131},
 primaryClass = "astro-ph.HE",
     year = 2015,
    month = mar,
   volume = 3,
      eid = {055},
    pages = {055},
      doi = {10.1088/1475-7516/2015/03/055},
}
@ARTICLE{Sys3,
   author = {{Actis}, M. and {Agnetta}, G. and {Aharonian}, F. and {Akhperjanian}, A. and 
	{Aleksi{\'c}}, J. and {Aliu}, E. and {Allan}, D. and {Allekotte}, I. and 
	{Antico}, F. and {Antonelli}, L.~A. and et al.},
    title = "{Design concepts for the Cherenkov Telescope Array CTA: an advanced facility for ground-based high-energy gamma-ray astronomy}",
  journal = {Experimental Astronomy},
   eprint = {1008.3703},
     year = 2011,
    month = dec,
   volume = 32,
    pages = {193-316},
      doi = {10.1007/s10686-011-9247-0},
}

@ARTICLE{2014Zampieri,
   author = {{Zampieri}, L. and {{\v C}ade{\v z}}, A. and {Barbieri}, C. and 
	{Naletto}, G. and {Calvani}, M. and {Barbieri}, M. and {Verroi}, E. and 
	{Zoccarato}, P. and {Occhipinti}, T.},
    title = "{Optical phase coherent timing of the Crab nebula pulsar with Iqueye at the ESO New Technology Telescope}",
  journal = {Monthly Notices of the Royal Astronomical Society},
archivePrefix = "arXiv",
   eprint = {1402.2571},
     year = 2014,
    month = apr,
   volume = 439,
    pages = {2813-2821},
      doi = {10.1093/mnras/stu136},
}
@ARTICLE{2016Ansoldi,
   author = {{Ansoldi}, S. and others},
    title = "{Teraelectronvolt pulsed emission from the Crab Pulsar detected by MAGIC}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1510.07048},
 primaryClass = "astro-ph.HE",
 keywords = {gamma rays: stars, pulsars: individual: Crab pulsar, stars: neutron},
     year = 2016,
    month = jan,
   volume = 585,
      eid = {A133},
    pages = {A133},
      doi = {10.1051/0004-6361/201526853},
}

@ARTICLE{2019APh...105...44S,
       author = {{Shilon}, I. and {Kraus}, M. and {B{\"u}chele}, M. and {Egberts}, K. and
         {Fischer}, T. and {Holch}, T.~L. and {Lohse}, T. and {Schwanke}, U. and
         {Steppa}, C. and {Funk}, S.},
        title = "{Application of deep learning methods to analysis of imaging atmospheric Cherenkov telescopes data}",
      journal = {Astroparticle Physics},
     keywords = {Gamma-ray astronomy, IACT, Analysis technique, Deep learning, Convolutional neural networks, Recurrent neural networks, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2019",
        month = "Feb",
       volume = {105},
        pages = {44-53},
          doi = {10.1016/j.astropartphys.2018.10.003},
archivePrefix = {arXiv},
       eprint = {1803.10698},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019APh...105...44S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2018arXiv181000592M,
       author = {{Mangano}, S. and {Delgado}, C. and {Bernardos}, M. and {Lallena}, M. and
         {Rodr{\'\i}guez V{\'a}zquez}, J.~J.},
        title = "{Extracting gamma-ray information from images with convolutional neural network methods on simulated Cherenkov Telescope Array data}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
         year = "2018",
        month = "Oct",
          eid = {arXiv:1810.00592},
        pages = {arXiv:1810.00592},
archivePrefix = {arXiv},
       eprint = {1810.00592},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018arXiv181000592M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2008Aliu,
   author = {{Aliu}, E. and others},
    title = "{Observation of Pulsed {$\gamma$}-Rays Above 25 GeV from the Crab Pulsar with MAGIC}",
  journal = {Science},
archivePrefix = "arXiv",
   eprint = {0809.2998},
     year = 2008,
    month = nov,
   volume = 322,
    pages = {1221},
      doi = {10.1126/science.1164718},
}

@ARTICLE{2017Dubner,
   author = {{Dubner}, G. and {Castelletti}, G. and {Kargaltsev}, O. and 
	{Pavlov}, G.~G. and {Bietenholz}, M. and {Talavera}, A.},
    title = "{Morphological Properties of the Crab Nebula: A Detailed Multiwavelength Study Based on New VLA, HST, Chandra, and XMM-Newton Images}",
  journal = {\apj},
     year = 2017,
    month = may,
   volume = 840,
      eid = {82},
    pages = {82},
      doi = {10.3847/1538-4357/aa6983},
}

@ARTICLE{2014Bridge,
   author = {{Aleksi{\'c}}, J. and others
	},
    title = "{Detection of bridge emission above 50 GeV from the Crab pulsar with the MAGIC telescopes}",
  journal = {\apj},
   eprint = {1402.4219},
      year = 2014,
    month = may,
   volume = 565,
      eid = {L12},
    pages = {L12},
      doi = {10.1051/0004-6361/201423664},
}


@ARTICLE{1985Davidson,
   author = {{Davidson}, K. and {Fesen}, R.~A.},
    title = "{Recent developments concerning the Crab Nebula}",
  journal = {Annual review of astronomy and astrophysics},
 keywords = {Crab Nebula, Ejecta, Supernova Remnants, Abundance, Astronomical Spectroscopy, Filaments, Morphology, Nebulae, Stellar Mass},
     year = 1985,
   volume = 23,
    pages = {119-146},
      doi = {10.1146/annurev.aa.23.090185.001003},
}

@ARTICLE{2016ctools,
   author = {{Kn{\"o}dlseder}, J. and {Mayer}, M. and {Deil}, C. and {Cayrou}, J.-B. and 
	{Owen}, E. and {Kelley-Hoskins}, N. and {Lu}, C.-C. and {Buehler}, R. and 
	{Forest}, F. and {Louge}, T. and {Siejkowski}, H. and {Kosack}, K. and 
	{Gerard}, L. and {Schulz}, A. and {Martin}, P. and {Sanchez}, D. and 
	{Ohm}, S. and {Hassan}, T. and {Brau-Nogu{\'e}}, S.},
    title = "{GammaLib and ctools. A software framework for the analysis of astronomical gamma-ray data}",
  journal = {Astronomy \& Astrophysics},
archivePrefix = "arXiv",
   eprint = {1606.00393},
 primaryClass = "astro-ph.IM",
 keywords = {methods: data analysis, virtual observatory tools},
     year = 2016,
    month = aug,
   volume = 593,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201628822},
}

@ARTICLE{Hester2008,
   author = {{Hester}, J.~J.},
    title = "{The Crab Nebula: An Astrophysical Chimera}",
  journal = {Annual Review of Astronomy \& Astrophysics},
     year = 2008,
    month = sep,
   volume = 46,
    pages = {127-155},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Buehler2012,
   author = {{Buehler}, R. and {Scargle}, J.~D. and {Blandford}, R.~D. and 
	{Baldini}, L. and {Baring}, M.~G. and {Belfiore}, A. and {Charles}, E. and 
	{Chiang}, J. and {D'Ammando}, F. and {Dermer}, C.~D. and {Funk}, S. and 
	{Grove}, J.~E. and {Harding}, A.~K. and {Hays}, E. and {Kerr}, M. and 
	{Massaro}, F. and {Mazziotta}, M.~N. and {Romani}, R.~W. and 
	{Saz Parkinson}, P.~M. and {Tennant}, A.~F. and {Weisskopf}, M.~C.
	},
    title = "{Gamma-Ray Activity in the Crab Nebula: The Exceptional Flare of 2011 April}",
  journal = {The Astrophysical Journal},
archivePrefix = "arXiv",
   eprint = {1112.1979},
     year = 2012,
    month = apr,
   volume = 749,
      eid = {26},
    pages = {26},
      doi = {10.1088/0004-637X/749/1/26},
}
@ARTICLE{Buhler2014,
   author = {{B{\"u}hler}, R. and {Blandford}, R.},
    title = "{The surprising Crab pulsar and its nebula: a review}",
  journal = {Reports on Progress in Physics},
     year = 2014,
    month = jun,
   volume = 77,
   number = 6,
      eid = {066901},
    pages = {066901},
      doi = {10.1088/0034-4885/77/6/066901},
}

@ARTICLE{Romoli2017,
   author = {{Romoli}, C. and {Taylor}, A.~M. and {Aharonian}, F.},
    title = "{Cut-off characterisation of energy spectra of bright fermi sources: Current instrument limits and future possibilities}",
  journal = {Astroparticle Physics},
archivePrefix = "arXiv",
   eprint = {1608.01501},
     year = 2017,
    month = feb,
   volume = 88,
    pages = {38-45},
      doi = {10.1016/j.astropartphys.2016.12.007},

}


@ARTICLE{Arons2012,
   author = {{Arons}, J.},
    title = "{Pulsar Wind Nebulae as Cosmic Pevatrons: A Current Sheet's Tale}",
  journal = {Space Science Reviews},
archivePrefix = "arXiv",
   eprint = {1208.5787},
     year = 2012,
    month = nov,
   volume = 173,
    pages = {341-367},
      doi = {10.1007/s11214-012-9885-1},
}

@ARTICLE{Cerutti:2016,
   author = {{Cerutti}, B. and {Philippov}, A.~A. and {Spitkovsky}, A.},
    title = "{Modelling high-energy pulsar light curves from first principles}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.01785},
     year = 2016,
    month = apr,
   volume = 457,
    pages = {2401-2414},
      doi = {10.1093/mnras/stw124},
}

@ARTICLE{kuiper2001,
   author = {{Kuiper}, L. and {Hermsen}, W. and {Cusumano}, G. and {Diehl}, R. and 
	{Sch{\"o}nfelder}, V. and {Strong}, A. and {Bennett}, K. and 
	{McConnell}, M.~L.},
    title = "{The Crab pulsar in the 0.75-30 MeV range as seen by CGRO COMPTEL. A coherent high-energy picture from soft X-rays up to high-energy gamma-rays}",
  journal = {\aap},
   eprint = {astro-ph/0109200},
     year = 2001,
    month = nov,
   volume = 378,
    pages = {918-935},
      doi = {10.1051/0004-6361:20011256},
}



@ARTICLE{Lyutikov:2012,
   author = {{Lyutikov}, M. and {Otte}, N. and {McCann}, A.},
    title = "{The Very High Energy Emission from Pulsars: A Case for Inverse Compton Scattering}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1108.3824},
 primaryClass = "astro-ph.HE",
 keywords = {gamma rays: stars, ISM: supernova remnants, pulsars: individual: Crab},
     year = 2012,
    month = jul,
   volume = 754,
      eid = {33},
    pages = {33},
      doi = {10.1088/0004-637X/754/1/33},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...754...33L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Cheng:1986,
   author = {{Cheng}, K.~S. and {Ho}, C. and {Ruderman}, M.},
    title = "{Energetic radiation from rapidly spinning pulsars. I - Outer magnetosphere gaps. II - VELA and Crab}",
  journal = {\apj},
     year = 1986,
    month = jan,
   volume = 300,
    pages = {500-539},
      doi = {10.1086/163829},
}



@ARTICLE{Aharonian2004,
   author = {{Aharonian}, F. and others},
    title = "{The Crab Nebula and Pulsar between 500 GeV and 80 TeV: Observations with the HEGRA Stereoscopic Air Cerenkov Telescopes}",
  journal = {The Astrophysical Journal},
   eprint = {astro-ph/0407118},
 keywords = {Acceleration of Particles, Gamma Rays: Observations, Gamma Rays: Theory, ISM: Individual: Name: Crab Nebula, pulsars: individual (Crab pulsar)},
     year = 2004,
    month = oct,
   volume = 614,
    pages = {897-913},
      doi = {10.1086/423931},
}


@ARTICLE{2017ICRCgammapy,
   author = {{Deil}, C. and others},
    title = "{Gammapy - A prototype for the CTA science tools}",
  journal = {International Cosmic Ray Conference},
archivePrefix = "arXiv",
   eprint = {1709.01751},
 primaryClass = "astro-ph.IM",
     year = 2017,
    month = jan,
   volume = 35,
      eid = {766},
    pages = {766},
}

@INPROCEEDINGS{2015ICRCgammapy,
   author = {{Donath}, A. and {Deil}, C. and {Arribas}, M.~P. and {King}, J. and 
	{Owen}, E. and {Terrier}, R. and {Reichardt}, I. and {Harris}, J. and 
	{Buehler}, R. and {Klepser}, S.},
    title = "{Gammapy: An open-source Python package for gamma-ray astronomy}",
booktitle = {34th International Cosmic Ray Conference (ICRC2015)},
     year = 2015,
   series = {International Cosmic Ray Conference},
   volume = 34,
archivePrefix = "arXiv",
   eprint = {1509.07408},
 primaryClass = "astro-ph.IM",
   editor = {{Borisov}, A.~S. and {Denisova}, V.~G. and {Guseva}, Z.~M. and 
	{Kanevskaya}, E.~A. and {Kogan}, M.~G. and {Morozov}, A.~E. and 
	{Puchkov}, V.~S. and {Pyatovsky}, S.~E. and {Shoziyoev}, G.~P. and 
	{Smirnova}, M.~D. and {Vargasov}, A.~V. and {Galkin}, V.~I. and 
	{Nazarov}, S.~I. and {Mukhamedshin}, R.~A.},
    month = jul,
      eid = {789},
    pages = {789},
}

@INPROCEEDINGS{Kirk2009,
   author = {{Kirk}, J.~G. and {Lyubarsky}, Y. and {Petri}, J.},
    title = "{The Theory of Pulsar Winds and Nebulae}",
booktitle = {Astrophysics and Space Science Library},
     year = 2009,
   series = {Astrophysics and Space Science Library},
   volume = 357,
   eprint = {astro-ph/0703116},
   editor = {{Becker}, W.},
    pages = {421},
      doi = {10.1007/978-3-540-76965-1_16},
   adsurl = {http://adsabs.harvard.edu/abs/2009ASSL..357..421K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Holler2015,
   author = {{Holler}, M. and {Berge}, D. and {van Eldik}, C. and {Lenain}, J.-P. and 
	{Marandon}, V. and {Murach}, T. and {de Naurois}, M. and {Parsons}, R.~D. and 
	{Prokoph}, H. and {Zaborov}, D. and {for the H.~E.~S.~S.~collaboration}
	},
    title = "{Observations of the Crab Nebula with H.E.S.S. Phase II}",
  journal = {ArXiv e-prints},
   eprint = {1509.02902},
     year = 2015,
    month = sep,
}




@ARTICLE{1969Natur.221..525C,
   author = {{Cocke}, W.~J. and {Disney}, M.~J. and {Taylor}, D.~J.},
    title = "{Discovery of Optical Signals from Pulsar NP 0532}",
  journal = {\nat},
     year = 1969,
    month = feb,
   volume = 221,
    pages = {525-527},
      doi = {10.1038/221525a0},
   adsurl = {http://adsabs.harvard.edu/abs/1969Natur.221..525C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@INPROCEEDINGS{2001Sherpa,
   author = {{Freeman}, P. and {Doe}, S. and {Siemiginowska}, A.},
    title = "{Sherpa: a mission-independent data analysis application}",
booktitle = {Astronomical Data Analysis},
     year = 2001,
   series = {Proc. SPIE},
   volume = 4477,
   eprint = {astro-ph/0108426},
   editor = {{Starck}, J.-L. and {Murtagh}, F.~D.},
    month = nov,
    pages = {76-87},
      doi = {10.1117/12.447161},
}

@InProceedings{SciPyProceedings,
  author =       {Brian L. Refsdal and Stephen M. Doe and Dan T. Nguyen and Aneta L. Siemiginowska and Nina R. Bonaventura and Douglas Burke and Ian N. Evans and Janet D. Evans and Antonella Fruscione and Elizabeth C. Galle and John C. Houck and Margarita Karovska and Nicholas P. Lee and Michael A. Nowak},
  title =        {Sherpa: 1D/2D modeling and fitting in Python},
  booktitle =   {Proceedings of the 8th Python in Science Conference},
  pages =     {51 - 57},
  address = {Pasadena, CA USA},
  year =      {2009},
  editor =    {Ga\"el Varoquaux and St\'efan van der Walt and Jarrod Millman},
}

@Manual{Rmanual,
  title = {R: A Language and Environment for Statistical Computing},
  author = {{R Core Team}},
  organization = {R Foundation for Statistical Computing},
  address = {Vienna, Austria},
  year = {2013},
  url = {http://www.R-project.org/},
}
@ARTICLE{1983LiMa,
   author = {{Li}, T.-P. and {Ma}, Y.-Q.},
    title = "{Analysis methods for results in gamma-ray astronomy}",
  journal = {Astrophysical Journal},
 keywords = {Gamma Ray Astronomy, Statistical Analysis, Confidence Limits, Maximum Likelihood Estimates, Monte Carlo Method},
     year = 1983,
    month = sep,
   volume = 272,
    pages = {317-324},
      doi = {10.1086/161295},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJ...272..317L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{2017HESSExtension,
   author = {{Holler}, M. and {Berge}, D. and {Hahn}, J. and {Khangulyan}, D. and 
	{Parsons}, R.~D. and {for the H.~E.~S.~S.~collaboration}},
    title = "{Advanced search for the extension of unresolved TeV sources with H.E.S.S.: First measurement of the extension of the Crab nebula at TeV energies}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1707.04196},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2017,
    month = jul,
   adsurl = {http://adsabs.harvard.edu/abs/2017arXiv170704196H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2017Burtovoi,
   author = {{Burtovoi}, A. and {Saito}, T.~Y. and {Zampieri}, L. and {Hassan}, T.
	},
    title = "{Prospects for the detection of high-energy (E > 25 GeV) Fermi pulsars with the Cherenkov Telescope Array}",
  journal = {Monthly Notices of the Royal Astronomical Society},
archivePrefix = "arXiv",
   eprint = {1706.07228},
 primaryClass = "astro-ph.HE",
 keywords = {pulsars: general, gamma-rays: stars},
     year = 2017,
    month = oct,
   volume = 471,
    pages = {431-446},
      doi = {10.1093/mnras/stx1582},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.471..431B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{1989Weekes,
   author = {{Weekes}, T.~C. and {Cawley}, M.~F. and {Fegan}, D.~J. and {Gibbs}, K.~G. and 
	{Hillas}, A.~M. and {Kowk}, P.~W. and {Lamb}, R.~C. and {Lewis}, D.~A. and 
	{Macomb}, D. and {Porter}, N.~A. and {Reynolds}, P.~T. and {Vacanti}, G.
	},
    title = "{Observation of TeV gamma rays from the Crab nebula using the atmospheric Cerenkov imaging technique}",
  journal = {Astrophysical Journal},
 keywords = {Cerenkov Counters, Crab Nebula, Gamma Ray Astronomy, Imaging Techniques, Pulsars, Azimuth, Electron Energy, Image Processing, Monte Carlo Method, Periodic Variations, Reflectors, Spectral Energy Distribution},
     year = 1989,
    month = jul,
   volume = 342,
    pages = {379-395},
      doi = {10.1086/167599},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...342..379W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1993Themistocle,
   author = {{THEMISTOCLE Collaboration} and {Baillon}, P. and {Behr}, L. and 
	{Danagoulian}, S. and {Dudelzak}, B. and {Espigat}, P. and {Eschstruth}, P. and 
	{Fabre}, B. and {Fontaine}, G. and {George}, R. and {Ghesquiere}, C. and 
	{Kovacs}, F. and {Meynadier}, C. and {Pons}, Y. and {Riskalla}, R. and 
	{Rivoal}, M. and {Roy}, P. and {Schune}, P. and {Socroun}, T. and 
	{Touchard}, A.~M. and {Vrana}, J.},
    title = "{Gamma ray spectrum of the Crab nebula in the multi TeV region k20}",
  journal = {Astroparticle Physics},
     year = 1993,
    month = dec,
   volume = 1,
    pages = {341-355},
      doi = {10.1016/0927-6505(93)90001-T},
}

@ARTICLE{2000Smith,
   author = {{Smith}, D.~A. and others
	},
    title = "{First Detection of Gamma Rays from the Crab Nebula with the CELESTE ``Solar Farm'' Cherenkov Detector}",
  journal = {Nuclear Physics B Proceedings Supplements},
     year = 2000,
    month = mar,
   volume = 80,
    pages = {163-172},
      doi = {10.1016/S0920-5632(99)00838-5},
}

@ARTICLE{2015Hassan,
   author = {{Hassan}, T. and {Arrabito}, L. and {Bernl{\"o}r}, K. and {Bregeon}, J. and 
	{Hinton}, J. and {Jogler}, T. and {Maier}, G. and {Moralejo}, A. and 
	{Di Pierro}, F. and {Wood}, M. and {CTA Consortium}, f.~t.},
    title = "{Second large-scale Monte Carlo study for the Cherenkov Telescope Array}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1508.06075},
      year = 2015,
    month = aug,

}

@ARTICLE{Gaia2016,
    author = {{Prusti}, T. and others},
    title = "{The Gaia mission}",
   journal = {Astronomy and Astrophysics},
   archivePrefix = "arXiv",
   eprint = {1609.04153},
   primaryClass = "astro-ph.IM",
   keywords = {space vehicles: instruments, Galaxy: structure, astrometry, parallaxes, proper motions, telescopes},
   year = 2016,
   month = nov,
   volume = 595,
   eid = {A1},
   pages = {A1},
   doi = {10.1051/0004-6361/201629272},
}
@book{universityphysics,
   author = {H. D. Young and R. A. Freedman},
   year = {2004},
   title = {University Physics with Modern Physics},
   edition = {11th edition},
   publisher = {Addison Wesley},
   address = {New York},
   page = {567}
}


@ARTICLE{2013CTA,
   author = {{Acharya}, B.~S. and {Actis}, M. and {Aghajani}, T. and {Agnetta}, G. and 
	{Aguilar}, J. and {Aharonian}, F. and {Ajello}, M. and {Akhperjanian}, A. and 
	{Alcubierre}, M. and {Aleksi{\'c}}, J. and et al.},
    title = "{Introducing the CTA concept}",
  journal = {Astroparticle Physics},
     year = 2013,
    month = mar,
   volume = 43,
    pages = {3-18},
      doi = {10.1016/j.astropartphys.2013.01.007},
}

@ARTICLE{Gaia2018,
   author = {{Brown}, A.~G.~A. and others},
   title = "{Gaia Data Release 2. Summary of the contents and survey properties}",
  journal = {Astronomy and Astrophysics},
  archivePrefix = "arXiv",
  eprint = {1804.09365},
  year = 2018,
  month = aug,
  volume = 616,
  eid = {A1},
  pages = {A1},
  doi = {10.1051/0004-6361/201833051},
}

@ARTICLE{Aleksic2015,
   author = {{Aleksi{\'c}}, J. and {Ansoldi}, S. and {Antonelli}, L.~A. and 
	{Antoranz}, P. and {Babic}, A. and {Bangale}, P. and {Barrio}, J.~A. and 
	{Becerra Gonz{\'a}lez}, J. and {Bednarek}, W. and {Bernardini}, E. and 
	{Biasuzzi}, B. and {Biland}, A. and {Blanch}, O. and {Bonnefoy}, S. and 
	{Bonnoli}, G. and {Borracci}, F. and {Bretz}, T. and {Carmona}, E. and 
	{Carosi}, A. and {Colin}, P. and {Colombo}, E. and {Contreras}, J.~L. and 
	{Cortina}, J. and {Covino}, S. and {Da Vela}, P. and {Dazzi}, F. and 
	{De Angelis}, A. and {De Caneva}, G. and {De Lotto}, B. and 
	{de O{\~n}a Wilhelmi}, E. and {Delgado Mendez}, C. and {Doert}, M. and 
	{Dominis Prester}, D. and {Dorner}, D. and {Doro}, M. and {Einecke}, S. and 
	{Eisenacher}, D. and {Elsaesser}, D. and {Fonseca}, M.~V. and 
	{Font}, L. and {Frantzen}, K. and {Fruck}, C. and {Galindo}, D. and 
	{Garc{\'{\i}}a L{\'o}pez}, R.~J. and {Garczarczyk}, M. and {Garrido Terrats}, D. and 
	{Gaug}, M. and {Godinovi{\'c}}, N. and {Gonz{\'a}lez Mu{\~n}oz}, A. and 
	{Gozzini}, S.~R. and {Hadasch}, D. and {Hanabata}, Y. and {Hayashida}, M. and 
	{Herrera}, J. and {Hildebrand}, D. and {Hose}, J. and {Hrupec}, D. and 
	{Idec}, W. and {Kadenius}, V. and {Kellermann}, H. and {Kodani}, K. and 
	{Konno}, Y. and {Krause}, J. and {Kubo}, H. and {Kushida}, J. and 
	{La Barbera}, A. and {Lelas}, D. and {Lewandowska}, N. and {Lindfors}, E. and 
	{Lombardi}, S. and {L{\'o}pez}, M. and {L{\'o}pez-Coto}, R. and 
	{L{\'o}pez-Oramas}, A. and {Lorenz}, E. and {Lozano}, I. and 
	{Makariev}, M. and {Mallot}, K. and {Maneva}, G. and {Mankuzhiyil}, N. and 
	{Mannheim}, K. and {Maraschi}, L. and {Marcote}, B. and {Mariotti}, M. and 
	{Mart{\'{\i}}nez}, M. and {Mazin}, D. and {Menzel}, U. and {Miranda}, J.~M. and 
	{Mirzoyan}, R. and {Moralejo}, A. and {Munar-Adrover}, P. and 
	{Nakajima}, D. and {Niedzwiecki}, A. and {Nilsson}, K. and {Nishijima}, K. and 
	{Noda}, K. and {Nowak}, N. and {Orito}, R. and {Overkemping}, A. and 
	{Paiano}, S. and {Palatiello}, M. and {Paneque}, D. and {Paoletti}, R. and 
	{Paredes}, J.~M. and {Paredes-Fortuny}, X. and {Persic}, M. and 
	{Prada Moroni}, P.~G. and {Prandini}, E. and {Preziuso}, S. and 
	{Puljak}, I. and {Reinthal}, R. and {Rhode}, W. and {Rib{\'o}}, M. and 
	{Rico}, J. and {Rodriguez Garcia}, J. and {R{\"u}gamer}, S. and 
	{Saggion}, A. and {Saito}, T. and {Saito}, K. and {Satalecka}, K. and 
	{Scalzotto}, V. and {Scapin}, V. and {Schultz}, C. and {Schweizer}, T. and 
	{Shore}, S.~N. and {Sillanp{\"a}{\"a}}, A. and {Sitarek}, J. and 
	{Snidaric}, I. and {Sobczynska}, D. and {Spanier}, F. and {Stamatescu}, V. and 
	{Stamerra}, A. and {Steinbring}, T. and {Storz}, J. and {Strzys}, M. and 
	{Takalo}, L. and {Takami}, H. and {Tavecchio}, F. and {Temnikov}, P. and 
	{Terzi{\'c}}, T. and {Tescaro}, D. and {Teshima}, M. and {Thaele}, J. and 
	{Tibolla}, O. and {Torres}, D.~F. and {Toyama}, T. and {Treves}, A. and 
	{Uellenbeck}, M. and {Vogler}, P. and {Wagner}, R.~M. and {Zanin}, R. and 
	{Horns}, D. and {Mart{\'{\i}}n}, J. and {Meyer}, M.},
    title = "{Measurement of the Crab Nebula spectrum over three decades in energy with the MAGIC telescopes}",
  journal = {Journal of High Energy Astrophysics},
archivePrefix = "arXiv",
   eprint = {1406.6892},
 primaryClass = "astro-ph.HE",
 keywords = {Crab Nebula, Pulsar wind nebulae, MAGIC telescopes, Imaging atmospheric Cherenkov telescopes, Very high energy gamma rays},
     year = 2015,
    month = mar,
   volume = 5,
    pages = {30-38},
      doi = {10.1016/j.jheap.2015.01.002},
   adsurl = {http://adsabs.harvard.edu/abs/2015JHEAp...5...30A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{magic_ecpl,
  author = {{MAGIC}, collaboration},
  journal = {personal communication},
  year = 2017
}
@article{Torres2014,
      author         = "Torres, Diego F. and Cillis, Anal{\'{\i}}a and Mart{\'{\i}}n, Jonatan
                        and de O{\~n}a Wilhelmi, Emma",
      title          = "{Time-dependent modeling of TeV-detected, young pulsar
                        wind nebulae}",
      journal        = "JHEAp",
      volume         = "1-2",
      year           = "2014",
      pages          = "31-62",
      doi            = "10.1016/j.jheap.2014.02.001",
      eprint         = "1402.5485",
      archivePrefix  = "arXiv",
      primaryClass   = "astro-ph.HE",
      SLACcitation   = "%%CITATION = ARXIV:1402.5485;%%"
}


@article{2010Meyer,
       author = {{Meyer}, M. and {Horns}, D. and {Zechlin}, H. -S.},
        title = "{The Crab Nebula as a standard candle in very high-energy astrophysics}",
      journal = {\aap},
         year = "2010",
        month = "Nov",
       volume = {523},
          eid = {A2},
        pages = {A2},
          doi = {10.1051/0004-6361/201014108},
archivePrefix = {arXiv},
       eprint = {1008.4524},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/\#abs/2010A&A...523A...2M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{1998Hillas,
	year = 1998,
	month = {aug},
	publisher = {{IOP} Publishing},
	volume = {503},
	number = {2},
	pages = {744--759},
	author = {A. M. Hillas and C. W. Akerlof and S. D. Biller and J. H. Buckley and D. A. Carter-Lewis and M. Catanese and M. F. Cawley and D. J. Fegan and J. P. Finley and J. A. Gaidos and F. Krennrich and R. C. Lamb and M. J. Lang and G. Mohanty and M. Punch and P. T. Reynolds and A. J. Rodgers and H. J. Rose and A. C. Rovero and M. S. Schubnell and G. H. Sembroski and G. Vacanti and T. C. Weekes and M. West and J. Zweerink},
	title = {The Spectrum of {TeV} Gamma Rays from the Crab Nebula},
	journal = {The Astrophysical Journal}
}

@article{Martin2012,
       author = {{Mart{\'\i}n}, Jonatan and {Torres}, Diego F. and {Rea}, Nanda},
        title = "{Time-dependent modelling of pulsar wind nebulae: study on the impact of the diffusion-loss approximations}",
      journal = {\mnras},
         year = "2012",
        month = "Nov",
       volume = {427},
        pages = {415-427},
          doi = {10.1111/j.1365-2966.2012.22014.x},
       eprint = {1209.0300},
}


@ARTICLE{KC84,
   author = {{Kennel}, C.~F. and {Coroniti}, F.~V.},
    title = "{Magnetohydrodynamic model of Crab nebula radiation}",
  journal = {\apj},
 keywords = {Crab Nebula, Magnetohydrodynamics, Stellar Models, Synchrotron Radiation, Spatial Distribution, Spectral Energy Distribution},
     year = 1984,
    month = aug,
   volume = 283,
    pages = {710-730},
      doi = {10.1086/162357},
   adsurl = {https://ui.adsabs.harvard.edu/abs/1984ApJ...283..710K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Hawc2019,
   author = {{HAWC Collaboration} and {Abeysekara}, A.~U. and {Albert}, A. and 
	{Alfaro}, R. and {Alvarez}, C. and {{\'A}lvarez}, J.~D. and 
	{Camacho}, J.~R.~A. and {Acero}, R. and {Arteaga-Vel{\'a}zquez}, J.~C. and 
	{Arunbabu}, K.~P. and {Avila Rojas}, D. and {Ayala Solares}, H.~A. and 
	{Baghmanyan}, V. and {Belmont-Moreno}, E. and {BenZvi}, S.~Y. and 
	{Brisbois}, C. and {Cabellero-Mora}, K.~S. and {Capistr{\'a}n}, T. and 
	{Carrami{\~n}ana}, A. and {Casanova}, S. and {Cotti}, U. and 
	{Cotzomi}, J. and {Couti{\~n}o de Le{\'o}n}, S. and {De la Fuente}, E. and 
	{de Le{\'o}n}, C. and {Dichiara}, S. and {Dingus}, B.~L. and 
	{DuVernois}, M.~A. and {D{\'{\i}}az-V{\'e}lez}, J.~C. and {Ellsworth}, R.~W. and 
	{Engel}, K. and {Espinoza}, C. and {Fick}, B. and {Fleischhack}, H. and 
	{Fraija}, N. and {Galv{\'a}n-G{\'a}mez}, A. and {Garc{\'{\i}}a-Gonz{\'a}lez}, J.~A. and 
	{Garfias}, F. and {Gonz{\'a}lez}, M.~M. and {Goodman}, J.~A. and 
	{Harding}, J.~P. and {Hernandez}, S. and {Hona}, B. and {Hueyotl-Zahuantitla}, F. and 
	{Hui}, C.~M. and {H{\"u}ntemeyer}, P. and {Iriarte}, A. and 
	{Jardin-Blicq}, A. and {Joshi}, V. and {Kaufmann}, S. and {Kieda}, D. and 
	{Lara}, A. and {Lee}, W.~H. and {Le{\'o}n Vargas}, H. and {Linnemann}, J.~T. and 
	{Longinotti}, A.~L. and {Luis-Raya}, G. and {Lundeen}, J. and 
	{Malone}, K. and {Marinelli}, S.~S. and {Martinez}, O. and {Martinez-Castellanos}, I. and 
	{Mart{\'{\i}}nez-Castro}, J. and {Mart{\'{\i}}nez-Huerta}, H. and 
	{Matthews}, J.~A. and {Miranda-Romagnoli}, P. and {Morales-Soto}, J.~A. and 
	{Moreno}, E. and {Mostaf{\'a}}, M. and {Nayerhoda}, A. and {Nellen}, L. and 
	{Newbold}, M. and {Nisa}, M.~U. and {Noriega-Papaqui}, R. and 
	{Peisker}, A. and {P{\'e}rez-P{\'e}rez}, E.~G. and {Pretz}, J. and 
	{Ren}, Z. and {Rho}, C.~D. and {Rivi{\`e}re}, C. and {Rosa-Gonz{\'a}lez}, D. and 
	{Rosenberg}, M. and {Ruiz-Velasco}, E. and {Salazar}, H. and 
	{Salesa Greus}, F. and {Sandoval}, A. and {Schneider}, M. and 
	{Schoorlemmer}, H. and {Seglar Arroyo}, M. and {Sinnis}, G. and 
	{Smith}, A.~J. and {Springer}, R.~W. and {Surajbali}, P. and 
	{Tabachnick}, E. and {Tanner}, M. and {Tibolla}, O. and {Tollefson}, K. and 
	{Torres}, I. and {Weisgarber}, T. and {Westerhoff}, S. and {Wood}, J. and 
	{Yapici}, T. and {Zepeda}, A. and {Zhou}, H.},
    title = "{Measurement of the Crab Nebula at the Highest Energies with HAWC}",
  journal = {arXiv e-prints},
   eprint = {1905.12518},
      year = 2019,
    month = may,
 }

    
}

@article{Lefa2012, 
 author = {{Lefa}, E. and {Kelner}, S.~R. and {Aharonian}, F.~A.},
    title = "{On the Spectral Shape of Radiation due to Inverse Compton Scattering Close to the Maximum Cutoff}",
  journal = {\apj},
   eprint = {1205.2929},
     year = 2012,
    month = jul,
   volume = 753,
      eid = {176},
    pages = {176},
      doi = {10.1088/0004-637X/753/2/176},
}

@article{Burnham2004,
author = {P Burnham, Kenneth and R Anderson, David},
year = {2004},
month = {01},
pages = {261-304},
title = {Multimodel Inference: understanding AIC and BIC in Model Selection},
volume = {33},
journal = {Sociological Methods Research}
}

@ARTICLE{Yeung2019,
       author = {{Yeung}, Paul K.~H. and {Horns}, Dieter},
        title = "{The Energy-dependent {\ensuremath{\gamma}}-Ray Morphology of the Crab Nebula Observed with the Fermi Large Area Telescope}",
      journal = {\apj},
     keywords = {gamma rays: ISM, ISM: individual objects: Crab Nebula, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Apr",
       volume = {875},
       number = {2},
          eid = {123},
        pages = {123},
          doi = {10.3847/1538-4357/ab107a},
archivePrefix = {arXiv},
       eprint = {1903.07527},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...875..123Y},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Bucciantini2011,
    author = {Bucciantini, N. and Arons, J. and Amato, E.},
    title = "{Modelling spectral evolution of pulsar wind nebulae inside supernova remnants}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {410},
    number = {1},
    pages = {381-398},
    year = {2010},
    month = {12},
    abstract = "{We present a new model for the spectral evolution of pulsar wind nebulae (PWNe) inside supernova remnants (SNRs). The model couples the long-term dynamics of these systems, as derived in the 1D approximation, with a one-zone description (all quantities are assumed uniform in the nebula) of the spectral evolution of the emitting plasma. Our goal is to provide a simplified theoretical description that can be used as a tool to put constraints on unknown properties of PWN-SNR systems: a piece of work that is preliminary to any more accurate and sophisticated modelling. In this paper, we apply the newly developed model to a few objects of different ages and luminosities. We find that an injection spectrum in the form of a broken power law gives a satisfactory description of the emission for all the systems we consider. More surprisingly, we also find that the intrinsic spectral break turns out to be at a similar energy for all sources, in spite of the differences mentioned above. We discuss the implications of our findings on the workings of pulsar magnetospheres, pair multiplicity and on the particle acceleration mechanism(s) that might be at work at the pulsar wind termination shock.}",
    issn = {0035-8711},
    doi = {10.1111/j.1365-2966.2010.17449.x},
    url = {https://doi.org/10.1111/j.1365-2966.2010.17449.x},
    eprint = {http://oup.prod.sis.lan/mnras/article-pdf/410/1/381/18446661/mnras0410-0381.pdf},
}


@ARTICLE{2010Tanaka,
       author = {{Tanaka}, S.~J. and {Takahara}, F.},
        title = "{A Model of the Spectral Evolution of Pulsar Wind Nebulae}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = "2010",
        month = "Jan",
          eid = {arXiv:1001.2360},
        pages = {arXiv:1001.2360},
archivePrefix = {arXiv},
       eprint = {1001.2360},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010arXiv1001.2360T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{Torres2013,
    author = {Torres, D. F. and Mart{\'\i}n, J. and de O{\~n}a Wilhelmi, E. and Cillis, Analia},
    title = "{The effects of magnetic field, age and intrinsic luminosity on Crab-like pulsar wind nebulae}",
    journal = {Monthly Notices of the Royal Astronomical Society},
    volume = {436},
    number = {4},
    pages = {3112-3127},
    year = {2013},
    month = {10},
    abstract = "{We investigate the time-dependent behaviour of Crab-like pulsar wind nebulae (PWNe) generating a set of models using four different initial spin-down luminosities (L0 = \\{1, 0.1, 0.01, 0.001\\} × L0,Crab), eight values of magnetic fraction (η = 0.001, 0.01, 0.03, 0.1, 0.5, 0.9, 0.99 and 0.999, i.e. from fully particle dominated to fully magnetically dominated nebulae) and three distinctive ages: 940, 3000 and 9000 years. We find that the self-synchrotron Compton (SSC) contribution is irrelevant for LSD = 0.1, 1 and 10 per cent of the Crab power, disregarding the age and the magnetic fraction. SSC only becomes relevant for highly energetic (∼70 per cent of the Crab), particle dominated nebulae at low ages (of less than a few kyr), located in a far-infrared (FIR) background with relatively low energy density. Since no pulsar other than Crab is known to have these features, these results clarify why the Crab nebula, and only it, is SSC dominated. No young PWN would be detectable at TeV energies if the pulsar's spin-down power is 0.1 per cent Crab or lower. For 1 per cent of the Crab spin-down, only particle-dominated nebulae can be detected by HESS-like telescopes when young enough (with details depending on the precise injection and environmental parameters). Above 10 per cent of the Crab's power, all PWNe are detectable by HESS-like telescopes if they are particle dominated, no matter the age. The impact of the magnetic fraction on the final spectral energy distribution is varied and important, generating order of magnitude variations in the luminosity output for systems that are otherwise the same (equal P, \\$\\dot\\{P\\}\\$, injection and environment).}",
    issn = {0035-8711},
    doi = {10.1093/mnras/stt1793},
    url = {https://doi.org/10.1093/mnras/stt1793},
    eprint = {http://oup.prod.sis.lan/mnras/article-pdf/436/4/3112/3081254/stt1793.pdf},
}


@ARTICLE{1973ApJ...186..249P,
       author = {{Pacini}, F. and {Salvati}, M.},
        title = "{On the Evolution of Supernova Remnants. Evolution of the Magnetic Field, Particles, Content, and Luminosity}",
      journal = {\apj},
         year = "1973",
        month = "Nov",
       volume = {186},
        pages = {249-266},
          doi = {10.1086/152495},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1973ApJ...186..249P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@article{Ackermann2018,
       author = { {Fermi-LAT Collaboration} and {Biteau}, J.},
        title = "{The Search for Spatial Extension in High-latitude Sources Detected by the Fermi Large Area Telescope}",
      journal = {Astrophysical Journal},
     keywords = {BL Lacertae objects: general, catalogs, gamma rays: general, ISM: H ii Regions, ISM: supernova remnants, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2018",
        month = "Aug",
       volume = {237},
       number = {2},
          eid = {32},
        pages = {32},
          doi = {10.3847/1538-4365/aacdf7},
archivePrefix = {arXiv},
       eprint = {1804.08035},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJS..237...32A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{2015Meagher,
       author = {{Meagher}, K. and {VERITAS Collaboration}},
        title = "{Six years of VERITAS observations of the Crab Nebula}",
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
    booktitle = {34th International Cosmic Ray Conference (ICRC2015)},
         year = "2015",
       series = {International Cosmic Ray Conference},
       volume = {34},
        month = "Jul",
          eid = {792},
        pages = {792},
archivePrefix = {arXiv},
       eprint = {1508.06442},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015ICRC...34..792M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2013deOna,
       author = {{De O{\~n}a-Wilhelmi}, E. and {Rudak}, B. and {Barrio}, J.~A. and
         {Contreras}, J.~L. and {Gallant}, Y. and {Hadasch}, D. and
         {Hassan}, T. and {Lopez}, M. and {Mazin}, D. and {Mirabal}, N. and
         {Pedaletti}, G. and {Renaud}, M. and {de los Reyes}, R. and
         {Torres}, D.~F. and {CTA Consortium}},
        title = "{Prospects for observations of pulsars and pulsar wind nebulae with CTA}",
      journal = {Astroparticle Physics},
     keywords = {Astrophysics - Instrumentation and Methods for Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2013",
        month = "Mar",
       volume = {43},
        pages = {287-300},
          doi = {10.1016/j.astropartphys.2012.08.009},
archivePrefix = {arXiv},
       eprint = {1209.0357},
 primaryClass = {astro-ph.IM},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013APh....43..287D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2011A&A...533A..10L,
       author = {{Lobanov}, A.~P. and {Horns}, D. and {Muxlow}, T.~W.~B.},
        title = "{VLBI imaging of a flare in the Crab nebula: more than just a spot}",
      journal = {Astronomy and Astrophysics},
     keywords = {ISM: supernova remnants, radio continuum: stars, pulsars: general, pulsars: individual: Crab pulsar, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2011",
        month = "Sep",
       volume = {533},
          eid = {A10},
        pages = {A10},
          doi = {10.1051/0004-6361/201117082},
archivePrefix = {arXiv},
       eprint = {1107.0182},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011A&A...533A..10L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2015Vigano,
       author = {{Vigan{\'o}}, Daniele and {Torres}, Diego F.},
        title = "{Modelling of the {\ensuremath{\gamma}}-ray pulsed spectra of Geminga, Crab, and Vela with synchro-curvature radiation}",
      journal = {Monthly Notices of the Royal Astronomical Society},
     keywords = {stars: neutron, gamma-rays: stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2015",
        month = "Jun",
       volume = {449},
       number = {4},
        pages = {3755-3765},
          doi = {10.1093/mnras/stv579},
archivePrefix = {arXiv},
       eprint = {1503.04060},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.449.3755V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Torres2018,
       author = {{Torres}, Diego F.},
        title = "{Order parameters for the high-energy spectra of pulsars}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena,
General Relativity and Quantum Cosmology},
         year = "2018",
        month = "Feb",
       volume = {2},
        pages = {247-256},
          doi = {10.1038/s41550-018-0384-5},
archivePrefix = {arXiv},
       eprint = {1802.04177},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018NatAs...2..247T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Torres2019,
       author = {{Torres}, Diego F. and {Vigan{\`o}}, Daniele and
         {Coti Zelati}, Francesco and {Li}, Jian},
        title = "{Synchrocurvature modelling of the multifrequency
non-thermal emission of pulsars}",
      journal = {Monthly Notices of the Royal Astronomical Society},
     keywords = {radiation mechanisms: non-thermal, stars: neutron,
Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Nov",
       volume = {489},
       number = {4},
        pages = {5494-5512},
          doi = {10.1093/mnras/stz2403},
archivePrefix = {arXiv},
       eprint = {1908.11574},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.489.5494T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Lyutikov2013,
       author = {{Lyutikov}, Maxim},
        title = "{Inverse Compton model of pulsar high-energy emission}",
      journal = {Monthly Notices of the Royal Astronomical Society},
     keywords = {pulsars: individual: Crab, gamma-rays: stars, X-rays:
stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2013",
        month = "May",
       volume = {431},
       number = {3},
        pages = {2580-2589},
          doi = {10.1093/mnras/stt351},
archivePrefix = {arXiv},
       eprint = {1208.5329},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013MNRAS.431.2580L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
